Small Changes, Big Impacts: Leveraging Diversity to Improve Energy Efficiency

In the last few years, a growing body of research has proposed methods, techniques, and tools to support developers in the construction of software that consumes less energy. These solutions leverage diverse approaches such as version history mining, analytical models, identifying energy-efficient color schemes, and optimizing the packaging of HTTP requests. In this chapter, we present a complementary approach. We advocate that developers should leverage software diversity to make software systems more energy-efficient. Our main insight is that non-specialists can build software that consumes less energy by alternating at development time between readily available, diversely-designed pieces of software implemented by third-parties. These pieces of software can vary in nature, granularity, and quality attributes. Examples include data structures and constructs for thread management and synchronization.

==> greenhub.tex <==

Addressing energy efficiency within mobile devices is particularly relevant as these devices have become one of our most used gadgets, and  most often run powered by batteries. As a consequence, battery life is a high priority concern for users and one of the major factors influencing consumer satisfaction~\cite{FRichter2018,thorwartConsumer}. On the other hand, battery life is also important for app developers, as excessive battery consumption is one of the most common causes for bad app reviews in app stores~\cite{fu2013people,khalid2015mobile}. 

As we have already witnessed in the previous section regarding the choice of data structures, developer decisions can directly impact the energy consumption of a mobile application (or simply ``app''). In general, when considering other factors such as location services~\cite{lin2010energy}, programming languages~\cite{Oliveira:2017},  color schemes~\cite{Vasquez:2018:MOO,Wan:2017}, or code refactorings~\cite{couto2020energy}, the use of one available solution over another can have non-negligible effect on energy consumption. 

Keeping energy usage to a minimum is so important for app developers that IDEs for the most popular smartphone platforms include energy profilers. 
However, profiling for energy within mobile environments is a particularly difficult problem, and particularly within Android, the mobile platform with the largest market share, and by a big margin.\footnote{https://gs.statcounter.com/os-market-share/mobile/worldwide} Indeed, Android is a highly heterogeneous platform: in 2015 there were already more than 24 thousand Android device models available,\footnote{https://www.zdnet.com/article/android-fragmentation-there-are-now-24000-devices-from-1300-brands/} and a recent study found out that there are more than 2.5 million apps in the Google Play Store.\footnote{https://www.statista.com/statistics/276623/number-of-apps-available-in-leading-app-stores/} In addition, the Android operating system is currently in its 10th major release, with multiple minor releases throughout the years. These numbers combined with the different ways in which apps and devices are used produce a virtually infinite number of potential usage scenarios.

In this context, profiling for energy consumption has only limited applicability. Alternatively, one needs to obtain large-scale information about energy use in real usage scenarios to make informed, effective decisions about energy optimization.
In this section, we describe how we leverage crowdsourcing to collect information about energy in real-world usage scenarios. We introduce the GreenHub initiative, \textbf{\url{https://greenhubproject.org/}}, which aims to promote collaboration as a path to produce the best energy-saving solutions. The most visible outcome of the initiative is a large dataset, called Farmer, that reflects \textit{in the wild}, real-world, usage of Android devices~\cite{matalonga2019greenhub}. 

The entries in Farmer include multiple pieces of information such as active sensors, memory usage, battery voltage and temperature, running applications, model and manufacturer, and network details. This raw data was obtained by continuous crowdsourcing through a mobile application called BatteryHub. The collected data is strictly, and by construction, anonymous so as to ensure the privacy of all the app users. Indeed, it is impossible to associate any data with the user who originated it. 
The data collected by BatteryHub is then uploaded to a remote server, where it is made publicly available to be used by third parties in research on improving the energy efficiency of apps, infrastructure software, and devices.

In order to foster the involvement of the community,
Farmer is available for download in raw format and can be accessed by means of a backend Web app that provides an overview of the data and makes it available through a REST API. The dataset can also be queried by means of LumberJack, a command-line tool for interacting with the REST API. 

Within the GreenHub initiative, we were so far able to collect a dataset which is \textit{sizable}. Thus far it comprises 48+ million unique samples. The dataset is also \textit{diverse}. It includes data stemming from 2.5k+ different brands, 15k+ smartphone models, from over 73 Android versions, across 211 countries.

In the remainder of this section, we describe in  detail the alternatives that we have implemented to allow the community to access the data within our dataset. The main motivation for the section is then to foster the engagement of the community in exploring the data we are providing, in this way contributing to increase the knowledge on how energy saving strategies can be realized within Android devices.
We therefore expect that this section is particularly interesting for researchers and/or practitioners focusing on mobile development, and that have a data mining mindset.

\subsection{A collaborative approach to Android energy consumption optimization}

The success of GreenHub is dependent on its data, and to keep such data coming in, we plan to give back to the community in concrete and valuable ways. In this section, we focus on the ways that the community can access the data we are collecting.

The initiative relies on an open-source technological platform\footnote{\url{https://github.com/greenhub-project}}, whose architecture overview is shown in Figure~\ref{fig:greenhubInfra}. This platform includes our data collection Android app called BatteryHub, a command-line application interface called Lumberjack, and the Farmer REST API for prototyping queries, dashboard interface, and database for storing data. These components are further defined in the following sub-sections.

\normalsize
\begin{figure}[tb]
\centering
\includegraphics[width=0.5\columnwidth]{images/greenhubInfra}
\caption{GreenHub platform architecture. }
\label{fig:greenhubInfra}	
\end{figure}

\subsubsection*{Data Collection} is provided by BatteryHub, an Android app whose development was inspired by Carat~\cite{oliner2013carat}. Initially, we forked Carat's open-source code to take advantage of the data collection and storage mechanisms. On top of that, we  updated its data model to consider more details on modern devices, such as NFC and Flashlight usage, for example. In the same spirit of Carat, BatteryHub is entirely open-source. In contrast with Carat, however, all our collected data is permanently and publicly available, so as to strongly encourage and help others in collaborating, inspecting and/or reusing any artifact that we have developed or collected. 


BatteryHub is available at Google's Play Store\footnote{\url{https://play.google.com/store/apps/details?id=com.hmatalonga.greenhub}}, and tracks the broadcast of system events, such as changes to the battery's state and, when such an event occurs, obtains a sample of the device's current state. 
Batteryhub either uses the official Android SDK or custom implementations for universal device compatibility support, and periodically communicates with the server application (over HTTP) to upload, and afterwards remove, the locally stored samples.
Each sample characterizes a wide range of aspects that may affect battery usage, such as sensor usage, temperature, and the list of running applications. 

It is important to mention that the data collected from each user is made anonymous by design.
Each installation of BatteryHub~is associated with a random unique identifier and no personal information, such as phone number, location, or IMEI, is collected. This means that it is (strictly) not possible to identify any BatteryHub user, nor is it possible to associate any data with the user from whom it originates. 

In regards to sample collection frequency, a new data measurement is collected (to be sent to our server) when the battery's state changes. In most cases, this translates to a sample being sent at each 1\% battery change (which accounts to 95\% of the time according to our data).
The app allows for configurable alerts, e.g. when the battery reaches a certain temperature. Our overarching goal is to use BatteryHub to give suggestions to users, based on their usage profiles, on how to reduce the energy consumption of their device.

Besides BatteryHub, our infrastructure includes four additional components, as depicted in Figure~\ref{fig:greenhubInfra}. We envision they can be used in different stages of mining our dataset, which are described in the remainder of this section.
Finally, our infrastructure also includes a web dashboard interface\footnote{\url{https://farmer.greenhubproject.org/}}
that provides access to up-to-date statistics about the collected samples.

\subsubsection*{Fast prototyping of queries}

can be made by using Farmer's REST API, which was designed as a means to quickly interface with and explore the dataset. As every request made to the API must be authenticated, users must first obtain an API key in order to access the data in this fashion\footnote{\url{https://docs.greenhubproject.org/api/getting-started.html}}.  
The API provides real-time, selective access to the dataset and one may query, e.g., all samples for a given brand or OS version. Since the API is designed according to the REST methodology, this allows us to incrementally add new data models to be reflected within the API itself as the data protocol evolves over time.
After an API key has been successfully generated, one may request his/her own user profile from the API:

{\small
\begin{verbatim}
farmer.greenhubproject.org/api/v1/me?api_token=yourTokenHere
\end{verbatim}
}

\noindent 
Every successful API response is a JSON formatted document, and in this case the server will reply with the user details, as shown next.

{\scriptsize
\begin{verbatim}
{   "data": {
        "id": XX,
        "name": "Your Name",
        "email": "your@email.com",
        "email_verified_at": "YYYY-MM-DD HH:MM:SS",
        "created_at": "Mon. DD, YYYY",
        "updated_at": "YYYY-MM-DD HH:MM:SS",
        "roles": [ ... ]   }   }
\end{verbatim}
}

\noindent
It is now possible to use the API, for example, to list devices:

{\small
\begin{verbatim}
farmer.greenhubproject.org/api/v1/devices?api_token=yourToken
\end{verbatim}
}

\noindent
This request can take additional parameters for \textit{page} and devices \textit{per page}. A full description of all the available parameters for each request can be found in the API Reference\footnote{\url{https://docs.greenhubproject.org/api-reference/}}. 

The expected response from the request above is as follows: 

{\scriptsize
\begin{verbatim}
{   "data": [
	    {   "brand": "asus",
            "created_at": "2017-10-28 02:51:09",
            "id": 2518,
            "is_root": false,
            "kernel_version": "3.1835+",
            "manufacturer": "asus",
            "model": "ASUS_X008D",
            "product": "WW_Phone",
            "os_version": "7.0",
            "updated_at": "2017-10-28 02:51:09"
        },  ... ],
    "links": { ... },
    "meta":  { ... }   }
\end{verbatim}
}

\noindent
To get more detailed information, e.g., about a particular device whose identifier is 123, it is possible to request its samples:


{\scriptsize
\begin{verbatim}
farmer.greenhubproject.org/api/v1/devices/123/samples?api_token=yourToken
\end{verbatim}
}

\iffalse
\begin{lstlisting}
{   "data": [
		{
			"app_version": 14,
			"battery_level": 0.99,
			"battery_state": "Discharging",
			"country_code": "Unknown",
			"created_at": "2017-10-25 18:17:37",
			"database_version": 3,
			"id": 98,
			"memory_active": 1025820,
			"memory_free": 1899508,
			"memory_inactive": 420244,
			"memory_user": 173044,
			"memory_wired": 0,
			"network_status": "WIFI",
			"screen_brightness": -1,
			"screen_on": true,
			"timestamp": "2017-10-25 18:04:34",
			"timezone": "Europe/Lisbon",
			"triggered_by": "android.intent.action.BATTERY_CHANGED",
			"updated_at": "2017-10-25 18:17:37"
		},
        ...
	],
	"links": {
		...
	},
	"meta": {
	    ...
	}
}
\end{lstlisting}
\fi

A complementary approach to interface with the API is to use its command-line application interface Lumberjack.
Using this tool, users can perform flexible, on-demand queries to the data repository, to support quick prototyping of data queries applying different filters and parameters. Furthermore, users can quickly fetch subsets of the data without the need to download a snapshot of the entire dataset. The following is an example of a Lumberjack query to obtain the list of Google brand devices:

{\scriptsize
\begin{verbatim}
  $ greenhub lumberjack devices brand:google -o googleDevices.json
\end{verbatim}
}

\noindent
The following example queries the dataset for samples whose model is nexus and that were uploaded before May 31st 2018: 

{\scriptsize
\begin{verbatim}
  $ greenhub lumberjack samples model:nexus -R ..2018-05-31     
\end{verbatim}
}


\subsubsection*{Extensive Mining}
can be conducted from 
the samples we collected, and which are accessible through Farmer. The dataset is available as a zip archive file, in CSV format\footnote{\url{https://farmer.greenhubproject.org/storage/dataset.7z}}, and also in Parquet\footnote{\url{http://parquet.apache.org}} binary format\footnote{\url{https://farmer.greenhubproject.org/storage/dataset.parquet.7z}}, which can be analyzed more efficiently than a plain text dump. 
The dataset is also available as a MariaDB relational database. The samples sent by BatteryHub are queued to be processed by a PHP server application built using the Laravel framework\footnote{\url{https://laravel.com/}}. Each sample is received as a JSON formatted string that is deconstructed and correctly mapped within the database. 

The (simplified) data model that we employ is shown in Figure~\ref{fig:datamodel}, where each box represents a table (or a CSV file) in the dataset. \textsf{Samples} is the most important of them, including multiple features of varied nature, e.g., the unique sample id, the timestamp for each sample, the state of the battery (charging or discharging), the level of charge of the battery, whether the screen was on or not, and the free memory on the device.

\textsf{App\_Processes} is the largest among the tables of the dataset, containing information about each running process in the device at the time the sample was collected, e.g., whether it was a service or an app running on the foreground, its name, and version. \textsf{Battery\_Details} provides battery-related information such as whether the device was plugged to a charger or not and the temperature of the battery. \textsf{Cpu\_Statuses} indicates the percentage of the CPU under use, the accumulated up time, and sleep time. 
\textsf{Devices} provides device-specific information, such as the model and manufacturer of the device and the version of the operating system running on it. \textsf{Network\_Details} groups network-related information, e.g., network operator and type,  whether the device is connected to a wifi network, and the strength of the wifi signal. The \textsf{Settings} table records multiple yes/no settings for services such as bluetooth, location, power saver mode, and nfc, among others. Finally, \textsf{Storage\_Details} provides multiple features related to the secondary storage of the device.

\begin{figure}[htb!]
\centering
\includegraphics[width=0.6\columnwidth]{images/datamodel.png}
\caption{Entity Relationship diagram of the dataset}
\label{fig:datamodel}	
\end{figure}



\begin{comment}

\textbf{other paper}
%%%%%%%%%%%%%%%%%%%%




As pointed out by recent work, mining software repositories by leveraging tools such as those available in UNIX operating system “allows the incremental construction of sophisticated and highly-efficient data processing pipelines”10.
A number of previous initiatives aiming at collecting information about energy usage in a crowdsourced manner have been devised. For example, Carat11 collects information about smartphone usage in order to identify energy bugs, situations where an app running on a device consumes much more energy than it usually does under the same circumstances in other devices. The work of Chon and colleagues12 leverages crowdsourced information to estimate the battery capacity of a smartphone when compared to a new one and provides hints for users to configure their phones to save energy. Guo et al.13 have performed intra device analysis independently of manufacturer and operating system versions to identify battery discharging patterns, types of mobile apps, and their energy consumption patterns. 
Compared to all previous initiatives, GreenHub has a more collaborative approach, since it was designed to be used by third parties and all the collected data is made publicly available. Furthermore, it gathers information about modern sensor utilization (e.g., NFC) and concerning the battery itself (e.g., electric current), which are neglected by previous work. The combination of these distinctive factors may potentiate further breadth studies, since possibly performed by members of the community other than us, as well as depth studies, since more data is available.
This article presents an overview of GreenHub, its architecture and components, and explains the dataset that we have built. The article also provides a first concrete example of how this data can be used to better understand energy usage in real-world scenarios: we have, for now, compared the battery charging/discharging patterns for the different manufacturers that are represented in our dataset, and how these patterns have evolved through different versions of the Android operative system.


In fact, 
battery life is known to be one of the major factors influencing the  satisfaction of mobile device users~\cite{thorwartConsumer}. A recent survey with 1,894 smartphone users in the US placed battery life as the most important factor impacting smartphone purchasing decisions~\cite{FRichter2018}. Battery life is such a growing concern that it has been hypothesized that 9 out of 10 users suffer from low battery anxiety~\cite{wsjBatteryAnxiety}. 
%and is under discussion as a potential clinical condition: \textit{nomophobia}, the fear of being without your mobile phone, in the Diagnostic and Statistical Manual of Mental Disorders~\cite{bragazzi2014proposal}.

Developers are also very concerned with the impact their applications have on battery life. Excessive battery consumption is one of the most common causes for bad app reviews in app stores~\cite{fu2013people,khalid2015mobile}. In fact, developers are aware of the battery consumption problem, and many times seek help in solving this, even if they rarely receive adequate advice~\cite{pinto2014mining,manotas2016empirical,pang2016programmers}. Mobile device manufacturers recognize this issue and have tried to offer help by publishing developer guides aimed at extending battery life\footnote{\url{https://developer.android.com/topic/performance/power/}}\footnote{\url{https://developer.android.com/guide/topics/location/battery}}\footnote{\url{https://developer.android.com/docs/quality-guidelines/building-for-billions-battery-consumption}}.



Reducing the energy that is consumed by mobile devices is also an important problem from a sustainability point of view. Indeed, the billions of phones that are in use these days have a considerable environmental footprint. Our digital consumption (that includes but is not limited to mobile device usage) is bound to have a greater impact on global warming than the aviation industry~\cite{harris2018}.



Despite its importance, optimizing, or even analyzing energy consumption for mobile devices is a difficult and labor-intensive task for both users and/or developers. Developers are using different monitoring tools~\cite{Nucci2017,Hu2017,cruz2017} according to specific needs, which often results in a non-systematized procedure and context-specific findings~\cite{li14greens,Li2016http,cruz2017,Oliveira:2019:REE}. Monitoring the energy consumed by an application often results in extensive tests under several different scenarios and devices~\cite{li2013calculating,linares2014mining,Jabbarvand2015}, both very time consuming and potentially requiring large initial investments. In addition, Android is an heterogeneous platform.
In 2015, there were already more than 24,000 Android device models available in the world~\cite{Tung2015}. A recent study found out that there are more than 2.7 million apps in the Google Play Store. The Android operating system is currently in its 10th major release, with multiple minor releases throughout the years. These numbers compound with the different ways in which apps and devices are used to produce a virtually infinite number of potential usage scenarios. 

For users, understanding the energy consumption of their devices is an even harder exercise. Their knowledge regarding the behavior of the hardware is limited to their own devices. \added{Furthermore, without the proper tools and skills, they cannot compare the energy behavior of the apps they use, nor observe how such apps perform on other devices or under specific settings and conditions.} Moreover, different usage contexts of the same app, e.g., within different OS versions and with different hardware components switched on, result in different energy behaviors. This has to be taken into account when performing any comparison.

\added{In this paper, we present a descriptive and qualitative empirical study through indirect observation of a large real-world representative dataset, of day-to-day usage of Android devices. The aim of our qualitative study is to highlight associations between various characteristics and tendencies within a smartphone's ecosystem (considering real-world interaction and varying usage profiles) and battery usage. Our qualitative empirical study provides rich contextual data to better help understand the current status and phenomenon between smartphone usage and battery consumption.}



\added{The dataset under descriptive and qualitative analysis was gathered as part of the GreenHub initiative\footnote{\url{https://greenhubproject.org/}}, a collaborative approach to Android energy consumption analysis.} Our vision is to provide developers, researchers, device manufacturers, users, and any interested party with a rich set of data on how mobile devices and the apps running on them behave and use resources. We believe this data can promote the analysis and identification of opportunities to optimize energy consumption in Android devices, for both developers and users. In the case of developers, this will trigger further analyses that are beyond the dataset itself. These may explore the potential energy gains that have, e.g., been proposed in the context of location services~\cite{lin2010energy}, contrast~\cite{linares2015optimizing}, color scheme~\cite{linares2015optimizing, wan2017detecting}, data structure~\cite{hasan2016energy, pereira2018jstanley, pinto2016comprehensive, Pereira:2016:IJC:2896967.2896968}, programming language~\cite{oliveira2017study,  pereira2017sle, couto2017towards, lima2016haskell}, network usage~\cite{Li2016http}, and API~\cite{linares2014mining} usage.

For our qualitative analysis, we present a detailed characterization of the data and information within our dataset. This characterization allows not only a better understanding of the collected data for people trying to understand energy patterns in mobile devices, but also for those who might see the \greenhub{} dataset as a potential basis for studies with different goals (not necessarily associated with energy and battery consumption) across a wide range of directions. Indeed, we argue that this data is both rich and diverse enough to support other analyses in the context of Android.

\added{After thoroughly detailing our \greenhub{} dataset, we analyze the data in order to answer (ARQ) a set of 15 different research questions (RQs) regarding the battery consumption of Android smart-phones according to different scenarios and characteristics, such as: what are the battery/discharge tendencies across different countries, devices, network operators or brands. This lead us to several interesting findings. For instance, we noticed that with each new Android major version battery consumption actually tended to improve, but only after a particular version. Also, we were able to identify potential anomalies within a popular Android application, and even gather results that defied common intuition.}

\added{In order to answer such questions, we defined a new battery charging/discharging metric to be used within our dataset, which maintains a notion of data periods originating from the same device. This metric, which we named \ppm{}, \added{or \textit{percentage-per-minute}}, was used for understanding how a wide range of factors impact the battery consumption of Android devices and for identifying common tendencies.} 

\added{\ppm{} is a numerical value, either positive \ppm{}$^{+}$ or negative \ppm{}$^{-}$ reflecting battery charge or discharge respectively, calculated based on battery percentage change within one minute. \ppm{} does not represent an absolute battery, energy, or efficiency metric, but the \textbf{tendency} a given scenario has on the charging/discharging of the battery. This metric factors in real-world human interaction, and aspects such as different user profiles across vastly different devices, brands, countries, battery settings, and application usage.} 


In order to illustrate the potential of our dataset, we will also be presenting new and diverging potential research paths, which spontaneously sprouted from our work and analysis. These research paths (RP) will be introduced, where appropriately, while we discuss the data and our initial studies and findings in the paper. \added{These RPs further complement the RQ presented in this paper, by focusing on more specific questions and findings, while also opening research paths to establish the causality of our highlighted associations and suggesting hypotheses which can be tested in analytical studies. We believe they are as equally promising to be addressed and should so in dedicated studies, either by fully, or partially (through means of combining other datasets), using our presented dataset or data present within the dataset}. Note that some of these prospective research avenues are not specifically aiming for energy/battery consumption research, but also other areas of research on Android devices. \added{For example, our data can help with research paths such as: how do new applications spread worldwide?; How frequent do users update their OS versions?; Is there a relationship between a country's average temperature and battery drain; etc,.}

Not only is our dataset completely public, open-source, and permanently available, but also, for reproducibility, all the tools and processes used to generate the results and information in this paper are also publicly available. This includes the \greenhub{} Pipeline based on Jupyter Notebooks and the Python Pandas library, which allows for human-readable documents to perform data analysis in a modular and easy to visualize manner. \added{This Pipeline performed all the data cleaning, processing, and analysis which produced the results and answers to our RQs within this paper.} 



\added{Finally, the work presented in this paper extends a prior work of ours~\cite{matalonga2019greenhub}, where we previously presented the \greenhub{} infrastructure, the dataset model, and quantified the collected samples. This prior work is presented in Section~\ref{sec:greenhub}, which we have added a more detailed explanation of how to access the data through our REST API, and examples of how to query the \farmer{} database. Additionally, this public dataset itself has been updated to contain half a year's worth of new data samples. The novel contributions include the detailed exploration of the dataset, study on the battery tendencies based on human-smartphone interactions, proposal of other research avenues based on this fruitful dataset, and an integrated data cleaning and analysis pipeline.}


To summarize, the main contributions of our research are:
\begin{enumerate}

    \item A detailed characterization of the \greenhub{} dataset, thus providing knowledge and understanding of the data in the dataset;
    \added{\item A qualitative empirical analysis of the collected human-smartphone interaction data to help identify the tendencies between battery charging/discharging of Android smartphones and various smartphone characteristics;}
    
    \item The proposal of several generic and energy/battery related research paths enabled by the data in the \greenhub{} dataset;
    
    \item A replication package consisting of the \greenhub{} Pipeline, for cleaning data, characterizing and querying the dataset, and analyzing battery charging/consumption tendencies.
\end{enumerate}

The remainder of this paper will describe: 
\begin{itemize}
    \item The setup and infrastructure for data collection, analysis, and storage \textbf{(Section~\ref{sec:greenhub})};
    \item A detailed characterization of the \greenhub{} dataset \textbf{(Sections~\ref{sec:empiricalstudy}} and \textbf{\ref{sec:batterydouble})};
%    \item A discussion and analysis on a peculiar situation regarding an app (Battery Double) which cloned ours (BatteryHub) \textbf{(Section~\ref{sec:batterydouble})}; \todo{fará sentido dar tanto destaque a este assunto?}
    \item An empirical study and results on the battery consumption tendencies of Android devices \textbf{(Section~\ref{sec:results})};
    \item The \greenhub{} Pipeline notebook replication package \textbf{(Section~\ref{sec:pipeline})};
    \added{\item A look at the threats to the validity of our study and results \textbf{(Section~\ref{sec:threats})};}
    \item Description of related work \textbf{(Section~\ref{sec:related})};
    \item Our conclusions and final comments of this paper \textbf{(Section~\ref{sec:conclusions})}.
\end{itemize}

%2) characterizacao detalhada para a comunidade usar
%4) estudo tendencias charge/discharge
%5) caminhos possiveis genericos e de energia
%6) pipeline reproduzivel 

\end{comment}
